Policy Stitching: Learning Transferable Robot Policies

Training robots with reinforcement learning (RL) typically involves heavy interactions with the environment, and the acquired skills are often sensitive to changes in task environments and robot kinematics. Transfer RL aims to leverage previous knowledge to accelerate learning of new tasks or new body configurations. However, existing methods struggle to generalize to novel robot-task combinations and scale to realistic tasks due to complex architecture design or strong regularization that limits the capacity of the learned policy. We propose Policy Stitching, a novel framework that facilitates robot transfer learning for novel combinations of robots and tasks. Our key idea is to apply modular policy design and align the latent representations between the modular interfaces. Our method allows direct stitching of the robot and task modules trained separately to form a new policy for fast adaptation. Our simulated and real-world experiments on various 3D manipulation tasks demonstrate the superior zero-shot and few-shot transfer learning performances of our method. Our project website is at: http://generalroboticslab.com/PolicyStitching/ .

==> sections/experiments.tex <==
\section{Experiments}

We aim to evaluate the performance of Policy Stitching (PS) in both zero-shot and few-shot transfer setups. Furthermore, we generalize our experiments to a physical robot setup to demonstrate the practical applicability and real-world performance. Finally, we provide quantitative and qualitative analysis to understand the role of the learned transferable representations in effective policy stitching.

\subsection{Simulation Experiment Setup and Baselines}

\begin{figure*}[t!]
\begin{center}
\centerline{\includegraphics[width=\textwidth]{Modularized Policy for Robot Transfer Learning - CoRL 2023/figures/task_robot.pdf}}
\caption{
\textbf{Simulation Experimental Setup}: From left to right, we show different task and robot configurations: standard table, slippery table, rough terrain with small rocks, cube object, stick object, 7-DoF Franka Emika Panda arm, third joint locked, and fifth joint locked.}
\label{fig:tasks_robots}
\end{center}
\vspace{-25pt}
\end{figure*}

We modify the panda-gym environment \cite{gallouedec2021pandagym} to simulate $5$ manipulation task environments and $3$ distinct robots with varying kinematics (Fig.\ref{fig:tasks_robots}). The tasks consist of $3$ push scenarios, where the robot must push a cube to the goal position on surfaces with very different friction properties, and $2$ pick tasks that involve pick and place task of objects with different shapes. In zero-shot evaluation, the stitched policy is directly tested without fine-tuning and each experiment consists of $200$ test trajectories, which are repeated $5$ times to report the mean and standard deviation. In few-shot evaluation, the stitched policy first interacts with the environment for additional $10$ epochs to store data in the replay buffer and is then fine-tuned for a few epochs with SAC. We train with $3$ random seeds to report the mean and standard deviation.

\textbf{Robot-Task Combination.} We evaluate PS on 8 robot-task combinations to cover policy stitching in both similar and dissimilar setup. We list all combinations as the titles of sub-figures in Fig.\ref{few_shot}. For instance, ``t: Pi1-R1'' represents a task module trained in the Pick1 task with Robot1, while ``r: Pu1-R2'' represents a robot module trained in the Push1 task with Robot2. These modules are then stitched together to form a new combination that has not been jointly trained together.

\textbf{Baselines.} We compare our method to the approach of \citet{devin2017learning}, which uses a similar modular policy but with small bottleneck and dropout as regularization to alleviate the modules misalignment issue. In the few-shot test, we also include an additional comparison to increase the bottleneck dimension of the \citet{devin2017learning}'s method to the same dimension as our method, since the original bottleneck dimension is too small to capture necessary information for complex 3D tasks. Furthermore, we provide an ablation study with our modular policy design but no latent representation alignment to study its importance. We also build a Plain baseline which is an MLP that takes in all the states at the first layer and has no modular structure. When transferring to novel task-robot combination, we split the Plain MLP network into two parts (i.e.,top-half and bottom-half) and perform the same reassembling operation as the modular networks. This operation that preserves a sub-network from the old task and adds a new sub-network for the new task has been widely used in other works \citep{huang2013cross, oquab2014learning, long2016unsupervised, yang2022evaluations, yoon2019scalable}. See Appendix \ref{apdx: network structure} for architecture details.

\textbf{Metrics.} We use success rate (task completion within a fixed number of steps) and touching rate (contact with the object during the task) as our evaluation metrics. In challenging transfer scenarios (e.g., a robot trained for a pushing task is required to perform a picking task), all methods may exhibit low success rates. Therefore, we use touching rate as a more informative metric to indicate whether the robot is engaging in meaningful interactions rather than arbitrary movements. Effective touching behavior can result in improved exploration for few-shot transfer learning, since touching serves as a preliminary behavior for picking or pushing.

\subsubsection{Results: Zero-Shot Transfer in Simulation}

\input{tables/zero_shot_table_ver9}

E1-E3 are easier robot-task combinations than E4-E8 since the unseen setup is closer to their original combinations. As shown in Tab.\ref{table:results_zeroshot_sim}, for E1-E3, PS achieves significantly better or comparable results than \citet{devin2017learning} and the PS(Ablation) method, suggesting the latent representation alignment serves as the fundamental step to enable effective module stitching. Our method also outperforms Plain MLP policy, which indicates both modular policy design and latent representation alignment are beneficial.

\begin{figure*}[b]
\vspace{-15pt}
\begin{center}
\centerline{\includegraphics[width=0.85\textwidth]{Modularized Policy for Robot Transfer Learning - CoRL 2023/figures/few-shot-plot-ver5.png}}
\vspace{-5pt}
\caption{\textbf{Success rates of the few-shot transfer learning in simulation. } 
}
\label{few_shot}
\end{center}
\vspace{-1.0cm}
\end{figure*}

For more challenging cases (E4-E8) where both task and robot configurations are drastically different, though all methods do not exhibit strong success rates, PS demonstrates notably higher touching rates. This implies more meaningful interactions that can potentially lead to a higher success rate and faster adaption in our few-shot experiments. Qualitatively, Plain baseline shows limited attempts to complete the task with frequent aimless arm swinging. Though PS(Ablation) and \citet{devin2017learning} methods show higher touching rates than the Plain baseline, they lack consistent attempts to move the target object to the goal after touching. In contrast, our PS method makes the robot attempt to push the object to the goal in most experiments. We show such qualitative comparisons in our supplementary video.

\subsubsection{Results: Few-shot Transfer in Simulation}

In Fig.\ref{few_shot}, PS achieves the highest or comparable success rates. Notably, in E2 and E4, while other methods tend to get stuck at local minima and reach a plateau at sub-optimal success rates, PS converges to significantly higher rates. In some experiments such as E1, E4, E5 and E7, PS transfers much faster and achieve higher success rates during the early phase of fine-tuning. This high transfer efficiency supports our hypothesis in the zero-shot experiment that the high touching rates achieved by PS can facilitate transfer learning through meaningful interactions. Even in challenging scenarios where all methods struggle to achieve a high success rate, PS can quickly adapt based on limited interactions. Furthermore, while some methods may achieve comparable results in a few instances, PS is the only method that demonstrates consistent satisfactory performance across all scenarios, suggesting that PS serves as a stable transfer learning framework.

\subsection{Real World Experiment}

First, we aim to evaluate the zero-shot transfer performance of PS in the real world by directly transferring the simulated policies to novel robot-task combinations. Moreover, we are interested in accessing the feasibility of continuously improving such policies given limited real-world interactions.

\begin{wrapfigure}[]{r}{0.35\textwidth}
\vspace{-18pt}
\begin{center} 
    \includegraphics[width=\linewidth]{Modularized Policy for Robot Transfer Learning - CoRL 2023/figures/real-world-setup.jpg}
\end{center}
\vspace{-10pt}
\caption{\textbf{Real World Setup}.}
\label{fig:real-world-setup}
\vspace{-13pt}
\end{wrapfigure}

\textbf{Setup.} In our real-world experiment (Fig.\ref{fig:real-world-setup}), we include a Robot1 as a 6-DoF UR5 arm, a Robot2 as the same UR5 arm but with the fifth joint being locked, a Task1 as pushing a cube to a goal position, and a Task2 as pushing a cylinder. The friction coefficient between the object and the table is 0.16 for Task 1 and 0.72 for Task 2. We first train Robot1-Task2 and Robot2-Task1 pairs in simulation. We then create Task1-Robot1 through policy stitching. For the few-shot experiments, we first fine-tune the policy for 50 epochs in simulation and test it in the real world. Following this, we then allow the policy to interact with the physical world for an additional 6 epochs (5 hours). We use an Intel RealSense D435i to detect the ArUco markers \citep{aruco2014} attached to the object and the goal position on the table. Both objects are 3D printed. The cylinder has a sandpaper at its bottom to increase the friction coefficient. All evaluation results are based on 20 testing instances.

\begin{wrapfigure}[]{r}{0.35\textwidth}
\vspace{-27pt}
\begin{center} 
    \includegraphics[width=\linewidth]{Modularized Policy for Robot Transfer Learning - CoRL 2023/figures/real-world-results.png}
\end{center}
\vspace{-10pt}
\caption{\textbf{Few-Shot Results}. Solid curves shown the fine-tuning in simulation. Dotted curves show the further fine-tuning in the real world.}
\label{fig:real-world-results}
\vspace{-15pt}
\end{wrapfigure}

\textbf{Zero-Shot Results.} PS achieves a success rate of \textbf{40\%} and a touching rate of \textbf{100\%} in zero-shot transfer. In comparison, both the PS(Ablation) method and the Plain baseline have 0\% success rate. The PS(Ablation) method achieves a 75\% touching rate, while the Plain baseline cannot even touch the object. The superior performances of PS indicate the great potential of policy stitching to generalize to novel robot-task combinations in real-world settings.

\textbf{Few-Shot Results.} As shown by the solid curves in Fig.\ref{fig:real-world-results}, after the first stage of fine-tuning in simulation, PS achieves the highest success rate of about 90\% in simulation, surpassing both the PS(Ablation) and Plain methods ($\sim$70\%). When this policy is directly transferred to the real UR5 arm, PS still achieves the highest success rate at 75\%, followed by the PS(Ablation) at 50\% and the Plain method at 45\%. 

These results indicate that the modular design with relative representation achieves a promising success rate on a new task in both simulation and the real world after a few epochs of fine-tuning. Due to the sim2real gap, the success rates of all methods drop to some extent. However, after 6 epochs of fine-tuning on the real robot platform shown as the dotted curves, PS results in a final success rate of 90\%. Although the success rates of both baselines (i.e., 60\% and 55\%) are improved after the fine-tuning, there is still a significant gap with the performance of PS. Through both zero-shot and few-shot experiments, we ensure that our method performs effectively, efficiently, and reliably in physical scenarios.

\subsection{Analysis: Latent Space at Module Interface}

\begin{figure}[t!]
\vspace{-20pt}
    \centering
  \begin{minipage}[b]{0.71\textwidth}
    \includegraphics[width=\linewidth]{figures/interface-analysis-ver2.png}
  \end{minipage}
  \begin{minipage}[b]{0.25\textwidth}
    \caption{\textbf{Latent Space Analysis.} We train robots with 3 different kinematics for the reaching task and visualize their latent space colorized by 4 groups of task states, similar to Fig.\ref{fig:teaser}. (A) Visualization of the 2D principal components of the latent representations. (B) The average pairwise cosine distances and L2 distances between each pair of the stitched latent states.}
    \label{fig:latent-space}
  \end{minipage}
% \label{fig:real-world-setup}
\vspace{-20pt}
\end{figure}

To understand how our latent space alignment benefits effective policy stitching by learning transferable representations, we provide further quantitative and qualitative analysis. Since the dimension of the latent embedding at the task-robot module interface is 128, we cannot directly visualize the latent representations. Therefore, we apply the Principal Component Analysis (PCA) \cite{pca} to reduce the dimension of the representation to 2. We train robots with 3 different kinematics on a reaching task with and without our latent space alignment. We colorize the principal components based on their task states and group them into four directions as in our motivation example in Fig.\ref{fig:teaser}(C). As shown in Fig.\ref{fig:latent-space}(A), the latent spaces of all policies trained with PS remain consistent across various training environments, while the latent spaces of policies trained without latent space alignment still show approximate isometric transformations. The consistent latent space explains the effectiveness of our policy stitching method.


To account for potential information loss during PCA visualization, we also provide quantitative analysis. In Fig.\ref{fig:latent-space}(B), we calculate the pairwise cosine distances and L2 distances (Appendix \ref{apdx:quant analysis interface}) between the raw high-dimensional latent states of different stitched policies. The pairwise distances are significantly smaller when the latent representations are aligned. PS achieves an average cosine distance of 0.0055 and L2 distance of 0.240, while ablation has a much higher cosine distance of 0.865 and L2 distance of 1.275. This analysis indicates that the latent representations of normal modular networks differ greatly from each other, and the latent representation alignment can successfully reduce such differences and facilitate the learning of transferable representations for policy stitching.

==> sections/method.tex <==
% modified from Easop version

% \begin{wrapfigure}{r}{0.45\textwidth}
% \vspace{-3.0cm}
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \centerline{\includegraphics[width=0.43\columnwidth]{figures/our_method.png}}
% % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% \end{center}
% \vspace{-0.5cm}
% \caption{our method.}
% \label{fig:our method}
% \vskip -0.2in
% \end{wrapfigure}

\section{Method: Policy Stitching}

\begin{figure}[t!]
\begin{center}
    \includegraphics[width=0.95\linewidth]{Modularized Policy for Robot Transfer Learning - CoRL 2023/figures/method_fig_ver6.png}
\end{center}
\vspace{-10pt}
\caption{\textbf{Method Overview.} Our modular policy design enables the task module to process task-specific states such as object states and environmental conditions and the robot module to process robot-specific states such as kinematics and dynamics. We generalize relative representations to model-free RL setup to align latent representations from separately trained policy networks. With both modular design and latent representation alignment, our method allows direct stitching of unseen combination of task and robot module for effective and efficient transfer.}
\vspace{-15pt}
\label{fig:method}
\end{figure}

Policy Stitching focuses on enabling effective knowledge transfer between different tasks or robot bodies. Our method consists of two main components: the modular policy design and transferable representations achieved through latent space alignment. Our framework is designed to be compatible with various model-free RL algorithms.

\subsection{Modular Policy Design}

% Traditional model-free RL policies have the benefit of end-to-end training. However, when it comes to transfer learning, the policy requires retraining of the entire network or certain selected layers. The selected layers are often treated as hyperparameters and are tuned through expensive trial and error. There is no guiding principle on how to conduct systematic transfer. To this end, 
% Pingcheng: similar meaning has been mentioned in inroduction?
We propose modular policy design to decompose the policy into two distinct modules focusing on robot specific and task specific information. Our design provides a straightforward ingredient for module reuse and stitching.

Consider an environment, $E$, with a robot $r$ and a presented task $k$, we formulate the problem as a Markov Decision Process with an observed state $s_E$ and action $a_E$. We denote the learning policy as $\pi_{E_{r k}}(a_E \mid s_E)$ which is parameterized by a function $\phi_{E_{r k}}(s_E)$. We utilize the model-free RL formulation in our experiments, specifically the Soft Actor-Critic (SAC) \citep{haarnoja2018soft} algorithm.

We decompose the state $s_E$, the policy function $\phi_{E_{r k}}(s_E)$, and the Q-function into a \textbf{robot-specific} module and a \textbf{task-specific} module (Fig. \ref{fig:method}). The state $s_E$ is decomposed into a robot-specific state $s_{E,\mathcal{R}}$ and a task-specific state $s_{E,\mathcal{T}}$. The robot-specific state $s_{E,\mathcal{R}}$ only consists of the joint angles of the robot, while the task-specific state $s_{E,\mathcal{T}}$ includes task information at hand such as the current position and orientation, linear and angular velocity, and goal position of the object. Similarly, the policy function $\phi_{E_{r k}}(s_E)$ is also decomposed into a task-specific module $g_k$ to encode the input task states, and a robot-specific module $f_r$ to implicitly capture robot kinematics and dynamics from input robot states. We follow the same design to  decompose the Q-function into task-specific module $q_k$ and robot-specific module $h_r$. Formally, our policy function and Q-function can be re-written as follows:
\begin{equation}
\phi_{E_{r k}}\left(s_E\right)=\phi_{E_{r k}}\left(s_{E, \mathcal{T}}, s_{E, \mathcal{R}}\right)=f_r\left(g_k\left(s_{E, \mathcal{T}}\right), s_{E, \mathcal{R}}\right).
\end{equation}
\begin{equation}
\begin{aligned}
Q_{E_{r k}}(s_E, a_E) = Q_{E_{r k}}\left(s_{E, \mathcal{T}}, s_{E, \mathcal{R}}, a_E\right)
=h_r\left(q_k\left(s_{E, \mathcal{T}}\right), s_{E, \mathcal{R}}, a_E\right),
\end{aligned}
\end{equation}

We name the modules after their main functionalities. Such modular design does not completely separate the information processing from each module. Since we train the entire policy end to end, the gradients flow in between the two modules during backpropagation. However, by explicitly enforcing their main functionalities through our modular design, we can still obtain effective improvements for robot transfer learning by reusing and stitching modules to leverage previously acquired knowledge. After the stitching, we can either use the new policy for zero-shot execution or perform few-shot learning for fast adaptation.

% For instance, if Robot A has acquired knowledge in performing Task X and Robot B has been trained for Task Y, we can transfer the learned task knowledge from Robot A to Robot B by simply stitching the task module related to Task X to the robot module representing Robot B. 

\subsection{Transferable Representations through Latent Space Alignment}

Our modular policy design allows for direct stitching, but a simple stitching approach may not yield optimal performance. Previous research \citep{devin2017learning} attributes the issue as overfitting to a particular robot and task, and has proposed to use dropout and very small bottleneck dimensions. However, the capacity of the policy is largely limited to simple 2D tasks and low-dimensional task states. Instead, we identify the fundamental issue as the lack of alignment enforcement of the latent embedding space at the output/input interface of two modules. Even under the same robot-task combination, the latent embedding vectors between the robot and task modules from different training seeds exhibit an almost isometric transformation relationship (Fig.\ref{fig:teaser}(B)). While similar observation has been made in supervised learning \citep{moschella2022relative, colah-blog}, we have identified and addressed this issue in the context of RL and demonstrate the effectiveness in knowledge transfer across novel robot-task combinations.

We propose to generalize Relative Representations \citep{moschella2022relative} in supervised learning to model-free RL. Unlike other techniques in supervised learning \citep{lenc2015understanding, gygli2021towards, hofmann2008kernel}, Relative Representations does not introduce additional learnable parameters. The key idea is to project all latent representations at the interface between two modules to a shared coordinate system among multiple policy networks. Through this invariance enforcement of transformation, we can establish a consistent latent representation of the task-state that aligns with the desired latent input of the robot module.

However, the original Relative Representations relies on the ground-truth labels in the supervised dataset to provide the anchor points for building the latent coordinate system. Our setup in RL does not come with such labels. The anchor points are analogous to the concept of basis in a linear system, hence should be as dissimilar from each other as possible. To overcome this challenge, we select an anchor set $\mathbb{A}$ from the training set $\mathbb{S}$ by leveraging the unsupervised clustering algorithm, k-means \cite{hartigan1979algorithm}, to identify the representative anchor points from the sampled task states. We select $k$ anchor states that are closest to the centroids of the clusters. The number of clusters $k$ depends on the dimension of the latent representation.

We want to represent every embedded task state $\boldsymbol{e}_{\boldsymbol{s}^{(i)}} = g_k\left(\boldsymbol{s}^{(i)}\right)$ with respect to the embedded anchor states $\boldsymbol{e}_{\boldsymbol{a}^{(j)}}=g_k\left(\boldsymbol{a}^{(i)}
\right)$, where $\boldsymbol{a}^{(j)} \in \mathbb{A}$ and $g_k$ is the task-specific module that embeds the task states. To this end, we capture the relationship between an embedded task state $\boldsymbol{e}_{\boldsymbol{s}^{(i)}}$ and an embedded anchor state $\boldsymbol{e}_{\boldsymbol{a}^{(j)}}$ using a similarity function $sim: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$, which calculates a similarity score $r=\operatorname{sim}\left(\boldsymbol{e}_{\boldsymbol{s}^{(i)}}, \boldsymbol{e}_{\boldsymbol{a}^{(j)}}\right)$. Given the anchor set $a^{(1)}, \ldots, a^{(|\mathbb{A}|)}$, the transferable representation of an input task state $\boldsymbol{s}^{(i)} \in \mathbb{S}$ is calculated by:
\begin{equation}
\begin{aligned}
\boldsymbol{r}_{\boldsymbol{s}^{(i)}} =
\left(\operatorname{sim}\left(\boldsymbol{e}_{\boldsymbol{s}^{(i)}}, \boldsymbol{e}_{\left.\boldsymbol{a}^{(1)}\right)}\right), \operatorname{sim}\left(\boldsymbol{e}_{\boldsymbol{s}^{(i)}}, \boldsymbol{e}_{\left.\boldsymbol{a}^{(2)}\right)}\right), 
\ldots, \operatorname{sim}\left(\boldsymbol{e}_{\boldsymbol{s}^{(i)}}, \boldsymbol{e}_{\left.\boldsymbol{a}^{(|A|)}\right)}\right)\right)
\end{aligned}
,
\end{equation}
which is a vector of length $|\mathbb{A}|$, and each element is the similarity score between the embedded task state and an embedded anchor state. We intentionally choose the cosine similarity as our similarity measure because it is invariant to isometric transformations. Although it is not invariant to vector translation, we add a normalization layer before calculating cosine similarity to mitigate this issue.

% : $\operatorname{sim}(\boldsymbol{a}, \boldsymbol{b})=\cos \theta=\frac{\boldsymbol{a} \boldsymbol{b}}{\|\boldsymbol{a}\|\|\boldsymbol{b}\|}$

\subsection{Implementation Details}

We challenge our methods in sparse reward setup and use hindsight experience replay \cite{andrychowicz2017hindsight} to encourage exploration. Both the task and robot modules are represented as MLPs \citep{haykin1998neural} with four layers and 256 hidden dimensions. The last layer of the task module and the first layer of the robot module have a dimension of 128, thus the dimension of the latent representation and the selected anchor set are also $128$ ($k=128$). Detailed network structures of our method and other baselines can be found in Appendix \ref{apdx: network structure}. Each of our policy is trained on $7$ threads of the AMD EPYC 7513 CPU and $1$ NVIDIA GeForce RTX 3090 GPU. Each training epoch consists of $35,000$ steps.

==> sections/regression.tex <==
\subsection{Information Preservation Test}
We are curious about how the communication problem happens. Is it because some important information is "forgotten" during its passing from one network module to another? Or all the key information is preserved when passed to another network module, but the succeeding network module cannot "understand" the information output in the format of the preceding network module?

To test these two hypotheses, we need to test whether the information that is important to the manipulation tasks still exist at the last layer of a reassembled policy network before the action mean value and standard deviation value are output. We choose the reassembled policy network of which the task module (top half of the baseline network) is trained in the Push1-Robot1 environment, and the robot module (bottom half of the baseline network) is trained in the Push2-Robot2 environment. We record the latent states output by the last layer, which are some $256$ dimensional vectors. We also record the corresponding object positions, goal positions, and end effector positions when these latent states are output.
\input{tables/regression.tex}
Then, we use the latent states as the data features, and the three positions as three kinds of labels, and do a regression on this dataset with a fully connected neural network. We use a simple $3$ layer fully connected network as the regression model, and adopt Adam \cite{kingma2014adam} as the optimization algorithm. We collect $10,000$ data points in total, using $8,000$ of them as the training set and $2,000$ of them as the testing set. As shown in Tabel \ref{regression}, all the three methods have nearly $100\%$ of success rates on the regression of the object position, goal position, and end effector position. The first two positions are input in the task state, while the end effector position is not directly given in the input, but requires be learned by the policy network according to the input joint angles and reward signal. The regression testing results show that the input object and goal position information is preserved till the last layer of the reassembled policy network. The learned robot kinematics is not only preserved in the robot module of our method and the ablation method, but also in the reassembled fully connected network of baseline.

Although the important information for robotic manipulation is preserved in the baseline network, the baseline policy cannot perform any reasonable attempts to accomplish the task, but always swings the robot arm in the air. These results suggest that the communication problem between different network modules is not caused by the "forgetting" of information, but by the failure of "understanding" the information passed from one network module to another.

==> tables/interface_motivation.tex <==
\begin{wraptable}{r}{0.66\textwidth}
% \centering
\footnotesize
\vspace{-0.5cm}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{random seed} & \multicolumn{1}{l|}{cosine distance} & \multicolumn{1}{l|}{L2 distance} & success rate \\ \hline
$101\&102$                         & $1.820$                                & $1.905$                            & $0.129\pm0.0208$ \\ \hline
$101\&103$                          & $1.437$                                & $1.693$                            & $0.222\pm0.0125$ \\ \hline

\end{tabular}
\caption{Success rates and distances.}
\vspace{-0.5cm}
\label{tab:motivation_stitching}
\end{wraptable} 

==> tables/main_pairwise_distance_table.tex <==
\begin{wraptable}{r}{0.55\textwidth}
\vspace{-1.0cm}
\footnotesize
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|l|}{}                                                    & cosine distance        & L2 distance          \\ \hline
\begin{tabular}[c]{@{}c@{}PS\end{tabular}    & $\mathbf{0.0055\pm0.0029}$ & $\mathbf{0.240\pm0.075}$ \\ \hline
\begin{tabular}[c]{@{}c@{}}PS(Ablation)\end{tabular} & $0.865\pm0.367$            & $1.275\pm0.311$          \\ \hline
\end{tabular}
\caption{Mean and standard deviation values of the average pairwise distances between different environment. They are calculated from the heat maps shown in Figure \ref{fig:latent-space}.}
\label{tab:main pairwise distance}
\vskip -0.2in
\end{wraptable} 

==> tables/main_pairwise_distance_table_ver2.tex <==

\begin{table}[h]
    \centering
    \fontsize{10}{12}\small
    \begin{tabular}{
        p{4cm}
        S[table-format=2.1]
        @{\extracolsep{50pt}}
        S[table-format=3.1]
        }
        \toprule
        \multicolumn{4}{c}{} & 
        \multicolumn{2}{c}{Metric}\\
        \cmidrule(lr){2-3}        
        Methods & {Cosine Distance} & {L2 Distance} 
        \\
        \midrule
        w/ relative representation     & $\boldsymbol{0.0055\pm0.0029}$ & $\boldsymbol{0.2400\pm0.0750}$  \\
        w/o relative representation &  $\math{0.8650\pm 0.3670}$      &     $\math{1.2750\pm 0.3110}$       \\

        \bottomrule
    \end{tabular}
    \caption{Mean and standard deviation of the average pairwise distances calculated from the heat maps in Fig.\ref{fig:latent-space}(B)}
    \label{table:real-zeroshot}
\end{table}

==> tables/main_pairwise_distance_table_ver3.tex <==
\begin{wraptable}{r}{0.53\textwidth}
% \footnotesize
\fontsize{10}{12}\small
\begin{tabular}{ccc}
\hline
Methods                     & Cosine Distance & L2 Distance \\ \hline
PS  & $\mathbf{0.0055\pm0.0029}$          & $\mathbf{0.240\pm0.075}$      \\
PS(Ablation) & $0.865\pm0.367$          & $1.275\pm0.311$      \\ \hline
\end{tabular}
\caption{Mean and standard deviation values of the average pairwise distances between different environment. They are calculated from the heat maps shown in Figure \ref{fig:latent-space}.}
\label{tab:main pairwise distance}
\vskip -0.2in
\end{wraptable} 

==> tables/real_zero_shot.tex <==
\begin{wraptable}{r}{0.46\textwidth}
\vspace{-1.4cm}
\small
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & ours             & ablation & baseline \\ \hline
success rate           & \textbf{40.0\%}  & 0.0\%    & 0.0\%    \\ \hline
touching rate          & \textbf{100.0\%} & 75.0\%   & 0.0\%    \\ \hline
\end{tabular}
\caption{Success rates and touching rates of the zero-shot transfer on real UR5 robot.}
\label{real zero shot}
\vskip -0.17in
\end{wraptable} 

==> tables/real_zero_shot_ver2.tex <==

\begin{table}[h]
    \centering
    \fontsize{10}{12}\small
    \begin{tabular}{
        p{3cm}
        S[table-format=2.1]
        @{\extracolsep{50pt}}
        S[table-format=3.1]
        }
        \toprule
        \multicolumn{4}{c}{} & 
        \multicolumn{2}{c}{Metric}\\
        \cmidrule(lr){2-3}        
        Methods & {Sucess Rate (\si{\percent})} & {Touching Rate (\si{\percent})} 
        \\
        \midrule
        Ours     & \textbf{40.0} & \textbf{100.0}  \\
        Ablation &  0.0          & 75.0            \\
        Baseline &  0.0          & 0.0             \\

        \bottomrule
    \end{tabular}
    \caption{Success rates and touching rates of the zero-shot transfer on real UR5 robot.}
    \label{table:real-zeroshot}
\end{table}

==> tables/real_zero_shot_ver3.tex <==
\begin{wraptable}{r}{0.50\textwidth}
\vspace{-0.5cm}
\centering
    \fontsize{10}{12}\small
    \begin{tabular}{ccc}
\hline
Methods  & Success Rate (\%) & Touching Rate (\%) \\ \hline
PS     & \textbf{40.0}     & \textbf{100.0}     \\
PS(Ablation) & 0.0               & 75.0               \\
Baseline & 0.0               & 0.0                \\ \hline
\end{tabular}
    \caption{\textbf{Success rates and touching rates of the zero-shot transfer on real UR5 arm.} Each data point is collected from $20$ games.}
    \label{table:real-zeroshot}
\vskip -0.25in
\end{wraptable} 

==> tables/regression.tex <==
\begin{table}[t]
\begin{tabular}{|l|l|l|l|l}
\cline{1-4}
                                                                & ours(\%) & ablation(\%) & baseline(\%) &  \\ \cline{1-4}
\begin{tabular}[c]{@{}l@{}}object\\ position\end{tabular}       & 99.65  & 100.00      & 100.00      &  \\ \cline{1-4}
\begin{tabular}[c]{@{}l@{}}goal\\ position\end{tabular}         & 99.10  & 99.90      & 100.00      &  \\ \cline{1-4}
\begin{tabular}[c]{@{}l@{}}end effector\\ position\end{tabular} & 99.75  & 100.00     & 100.00      &  \\ \cline{1-4}
\end{tabular}
\caption{Success rate of the regression test.}
\label{regression}
\end{table}

==> tables/zero_shot_table_ver2.tex <==
\begin{table}[]
\centering
% \begin{tabularx}{\textwidth}{|llllllll|}
\small
\begin{tabularx}{\textwidth}{|llllllll|}
\hline
        &                                                                                    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method with \\ relative representation\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method w/o\\ relative representation\end{tabular}} & \multicolumn{2}{c|}{baseline method} \tabularnewline
        &                                                                                    & Success (\%)                                       & Touching(\%)                                      & Success(\%)                             & Touching(\%)                                               & Success(\%)      & Touching(\%)      \tabularnewline \hline
Expt. 1 & \begin{tabular}[c]{@{}l@{}}task: Push1-Robotl \\ robot: Push2-Robot2\end{tabular}  & 26.9 + 3.6                                         & 73.0 + 1.4                                        & 13.9 + 3.5                              & \multicolumn{1}{l|}{75.8 4 4.4}                            & 6.5 + 2.5        & 0.0 + 0.0         \tabularnewline \hline
Expt. 2 & \begin{tabular}[c]{@{}l@{}}task: Push2-Robotl \\ robot: Push 1-Robot2\end{tabular} & 24.4 + 1.5                                         & 99.9 + 0.2                                        & 6.8 + 0.7                               & \multicolumn{1}{l|}{93.5 + 2.0}                            & 9.3 + 2.1        & 17.9 + 2.7        \tabularnewline \hline
Expt. 3 & \begin{tabular}[c]{@{}l@{}}task: Pushl-Robot3 \\ robot: Push3-Robot\end{tabular}   & 16.5 + 1.9                                         & 90.8 + 2.3                                        & 7.2 + 1.5                               & \multicolumn{1}{l|}{95.6 + 0.8}                            & 8.4 + 3.7        & 0.0 + 0.0         \tabularnewline \hline
Expt. 4 & \begin{tabular}[c]{@{}l@{}}task: Push3-Robotl \\ robot: Push 1-Robot2\end{tabular} & 13.2 + 1.1                                         & 95.4 + 1.9                                        & 14.9 + 1.0                              & \multicolumn{1}{l|}{88.7 + 1.1}                            & 9.0 + 1.4        & 1.6 + 1.0         \tabularnewline \hline
Expt. 5 & \begin{tabular}[c]{@{}l@{}}task: Pick 1-Robot \\ robot: Push 1-Robot2\end{tabular} & 2.1 + 0.4                                          & 14.7 + 2.7                                        & 4.0 + 1.9                               & \multicolumn{1}{l|}{9.6 + 1.6}                             & 3.8 + 1.6        & 2.8 + 0.9         \tabularnewline \hline
Expt. 6 & \begin{tabular}[c]{@{}l@{}}task: Push 1-Robot3 \\ robot: Pick1-Robot2\end{tabular} & 8.8 + 1.9                                          & 55.6 + 2.4                                        & 11.6 + 2.0                              & \multicolumn{1}{l|}{80.8 + 3.4}                            & 9.0 + 0.7        & 0.1 + 0.2         \tabularnewline \hline
Expt. 7 & \begin{tabular}[c]{@{}l@{}}task: Pick2-Robot \\ robot: Pick 1-Robot3\end{tabular}  & 4.7 + 1.6                                          & 41.8 + 1.7                                        & 3.6 + 0.8                               & \multicolumn{1}{l|}{13.1 + 2.9}                            & 3.2 + 1.4        & 0.0 + 0.0         \\ \hline
Expt. 8 & \begin{tabular}[c]{@{}l@{}}task: Pickl-Robot3 \\ robot: Pick2-Robotl\end{tabular}  & 5.3 + 1.7                                          & 18.4 + 1.3                                        & 3.0 I 0.7                               & \multicolumn{1}{l|}{18.8 + 2.6}                            & 3.0 + 0.7        & 0.0 + 0.0         \tabularnewline \hline
\end{tabularx}
\end{table}

==> tables/zero_shot_table_ver3.tex <==
\begin{table}
  \centering
  \renewcommand{\arraystretch}{1.2}
  \small
  \begin{tabular}{|p{3cm}|c|c|c|c|c|c|}
    \hline
    { } & \multicolumn{2}{c|}{\textbf{Our method}} & \multicolumn{2}{c|}{\textbf{ablation method}} & \multicolumn{2}{c|}{\textbf{baseline method}}\\
    % \hline
    % \textbf{Inactive Modes} & \textbf{Description}\\
    \cline{2-7}
    & \textbf{Success (\%)} & \textbf{Touching(\%)} & \textbf{Success(\%)} & \textbf{Touching(\%)} & \textbf{Success(\%)} & \textbf{Touching(\%)}\\
    %\hhline{~--}
    \hline
    \begin{tabular}{@{}c@{}}task: Push1-Robot1\\robot: Push2-Robot2\end{tabular} & $\mathbf{26.9\pm3.6}$ & $73.0\pm1.4$ & $13.9\pm3.5$ & $\mathbf{75.8\pm4.4}$ & $6.5\pm2.5$ & $0.0\pm0.0$\\ \hline
    \begin{tabular}{@{}c@{}}task: Push2-Robot1\\robot: Push1-Robot2\end{tabular} & $\mathbf{24.4\pm1.5}$ & $\mathbf{99.9\pm0.2}$ & $6.8\pm0.7$ & $93.5\pm2.0$ & $9.3\pm2.1$ & $17.9\pm2.7$\\ \hline
    \begin{tabular}{@{}c@{}}task: Push1-Robot3\\robot: Push3-Robot1\end{tabular} & $\mathbf{16.5\pm1.9}$ & $90.8\pm2.3$ & $7.2\pm1.5$ & $\mathbf{95.6\pm0.8}$ & $8.4\pm3.7$ & $0.0\pm0.0$\\ \hline
    \begin{tabular}{@{}c@{}}task: Push3-Robot1\\robot: Push1-Robot2\end{tabular} & $13.2\pm1.1$ & $\mathbf{95.4\pm1.9}$ & $\mathbf{14.9\pm1.0}$ & $88.7\pm1.1$ & $9.0\pm1.4$ & $1.6\pm1.0$\\ \hline
    \begin{tabular}{@{}c@{}}task: Pick1-Robot1\\robot: Push1-Robot2\end{tabular} & $2.1\pm0.4$ & $\mathbf{14.7\pm2.7}$ & $\mathbf{4.0\pm1.9}$ & $9.6\pm1.6$ & $3.8\pm1.6$ & $2.8\pm0.9$\\ \hline
    \begin{tabular}{@{}c@{}}task: Push1-Robot3\\robot: Pick1-Robot2\end{tabular} & $8.8\pm1.9$ & $55.6\pm2.4$ & $\mathbf{11.6\pm2.0}$ & $\mathbf{80.8\pm3.4}$ & $9.0\pm0.7$ & $0.1\pm0.2$\\ \hline
    \begin{tabular}{@{}c@{}}task: Pick2-Robot1\\robot: Pick1-Robot3\end{tabular} & $\mathbf{4.7\pm1.6}$ & $\mathbf{41.8\pm1.7}$ & $3.6\pm0.8$ & $13.1\pm2.9$ & $3.2\pm1.4$ & $0.0\pm0.0$\\ \hline
    \begin{tabular}{@{}c@{}}task: Pick1-Robot3\\robot: Pick2-Robot1\end{tabular} & $\mathbf{5.3\pm1.7}$ & $18.4\pm1.3$ & $3.0\pm0.7$ & $\mathbf{18.8\pm2.6}$ & $3.0\pm0.7$ & $0.0\pm0.0$\\ \hline
  \end{tabular}
  \caption{Success rate and touching rate of zero-shot transfer}
  \label{zero_shot_rates}
\end{table}

==> tables/zero_shot_table_ver5.tex <==
\begin{table}[h]
\centering
\small
\scalebox{0.9}{
\begin{tabular}{|cccccccc|}
\hline
        &                                                                                    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method with \\ relative representation\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method w/o\\ relative representation\end{tabular}} & \multicolumn{2}{c|}{baseline method} \\
        &                                                                                    & Success (\%)                                       & Touching(\%)                                      & Success(\%)                             & Touching(\%)                                               & Success(\%)      & Touching(\%)      \\ \hline
E. 1 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R1 \\ robot: Pu2-R2\end{tabular}  & $26.9\pm3.6$                                         & $73.0\pm1.4$                                        & $13.9\pm3.5$                              & \multicolumn{1}{lV{3}}{75.8\pm4.4}                            & $6.5\pm2.5$        & $0.0\pm0.0$         \\[0.3cm]
E. 2 & \begin{tabular}[c]{@{}l@{}}task: Pu2-R1 \\ robot: Pu1-R2\end{tabular} & $24.4\pm1.5$                                        & $99.9\pm0.2$                                       & $6.8\pm0.7$                               & \multicolumn{1}{lV{3}}{$93.5\pm2.0$}                            & $9.3\pm2.1$        & $17.9\pm2.7$        \\ [0.3cm]
E. 3 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R3 \\ robot: Pu3-R1\end{tabular}   & $16.5\pm1.9$                                         & $90.8\pm2.3$                                        & $7.2\pm1.5$                               & \multicolumn{1}{lV{3}}{$95.6\pm0.8$}                            & $8.4\pm3.7$        & $0.0\pm0.0$         \\ [0.3cm] \hlineB{3}
E. 4 & \begin{tabular}[c]{@{}l@{}}task: Pu3-R1 \\ robot: Pu1-R2\end{tabular} & $13.2\pm1.1$                                         & $95.4\pm1.9$                                        & $14.9\pm1.0$                              & \multicolumn{1}{lV{3}}{$88.7 \pm 1.1$}                            & $9.0 \pm 1.4$        & $1.6 \pm 1.0$         \\ [0.3cm]
E. 5 & \begin{tabular}[c]{@{}l@{}}task: Pi1-R1 \\ robot: Pu1-R2\end{tabular} & $2.1 \pm 0.4$                                          & $14.7 \pm 2.7$                                        & $4.0 \pm 1.9$                               & \multicolumn{1}{lV{3}}{$9.6 \pm 1.6$}                             & $3.8 \pm 1.6$        & $2.8 \pm 0.9$         \\ [0.3cm]
E. 6 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R3 \\ robot: Pi1-R2\end{tabular} & $8.8 + 1.9$                                          & $55.6 \pm 2.4$                                        & $11.6 \pm 2.0$                              & \multicolumn{1}{lV{3}}{$80.8 \pm 3.4$}                            & $9.0 \pm 0.7$        & $0.1 \pm 0.2$         \\ [0.3cm]
E. 7 & \begin{tabular}[c]{@{}l@{}}task: Pi2-R1 \\ robot: Pi1-R3\end{tabular}  & $4.7 \pm 1.6$                                          & $41.8 \pm 1.7$                                        & $3.6 \pm 0.8$                               & \multicolumn{1}{lV{3}}{$13.1 \pm 2.9$}                            & $3.2 \pm 1.4$        & $0.0 \pm 0.0$         \\ [0.3cm]
E. 8 & \begin{tabular}[c]{@{}l@{}}task: Pi1-R3 \\ robot: Pi2-R1\end{tabular}  & $5.3 \pm 1.7$                                          & $18.4 \pm 1.3$                                        & $3.0 \pm 0.7$                               & \multicolumn{1}{lV{3}}{$18.8 \pm 2.6$}                            & $3.0 \pm 0.7$        & $0.0\pm0.0$         \\ \hline

\end{tabular}}
\caption{Success rate and touching rate of zero-shot transfer. Our method with relative representation, without relative representation, and the baseline method use the network structures shown in Figure \ref{fig:ours structure}, \ref{fig:ablation structure}, \ref{fig:baseline structure} respectively. The success rate shows the probability of the robot to successfully accomplish the tasks, while the touching rate shows its probability touch the object in the tasks. The first three experiments are easier because the target tasks are easier and the source and target tasks are more similar. In these easier experiments our method achieves significantly higher success rates and touching rates than the baseline. In the other five harder experiments, all the methods have similarly low success rates, but our method still achieves higher touching rates than the baseline.}
\label{zero_shot_rates}
\vskip -0.5cm
\end{table}

==> tables/zero_shot_table_ver6.tex <==
\begin{table}[h]
\footnotesize
\centering
% https://tex.stackexchange.com/questions/39435/how-can-i-center-a-too-wide-table
\addtolength{\leftskip} {-2cm} % increase (absolute) value if needed
\addtolength{\rightskip}{-2cm}
\small
\scalebox{0.9}{
\begin{tabular}{|cccccccccc|}
\hline
        &                                                                                    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method with \\ relative representation\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}our method w/o\\ relative representation\end{tabular}} & \multicolumn{2}{c}{Devin et. al. 2017} & \multicolumn{2}{c|}{baseline method} \\
        &                                                                                    & Success (\%)                                       & Touching(\%)                                      & Success(\%)                             & Touching(\%)                                               & Success(\%)      & Touching(\%) & Success(\%)      & Touching(\%)      \\ \hline
E. 1 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R1 \\ robot: Pu2-R2\end{tabular}  & $26.9\pm3.6$                                         & $73.0\pm1.4$                                        & $13.9\pm3.5$                              & \multicolumn{1}{lV{3}}{75.8\pm4.4}                            & $11.7\pm2.6$        & $44.8\pm3.1$ & $6.5\pm2.5$        & $0.0\pm0.0$         \\[0.3cm]
E. 2 & \begin{tabular}[c]{@{}l@{}}task: Pu2-R1 \\ robot: Pu1-R2\end{tabular} & $24.4\pm1.5$                                        & $99.9\pm0.2$                                       & $6.8\pm0.7$                               & \multicolumn{1}{lV{3}}{$93.5\pm2.0$}                            & $10.0\pm0.9$        & $78.3\pm5.4$ & $9.3\pm2.1$        & $17.9\pm2.7$        \\ [0.3cm]
E. 3 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R3 \\ robot: Pu3-R1\end{tabular}   & $16.5\pm1.9$                                         & $90.8\pm2.3$                                        & $7.2\pm1.5$                               & \multicolumn{1}{lV{3}}{$95.6\pm0.8$}                            & $9.8\pm2.5$        & $82.6\pm1.6$ & $8.4\pm3.7$        & $0.0\pm0.0$         \\ [0.3cm] \hlineB{3}
E. 4 & \begin{tabular}[c]{@{}l@{}}task: Pu3-R1 \\ robot: Pu1-R2\end{tabular} & $13.2\pm1.1$                                         & $95.4\pm1.9$                                        & $14.9\pm1.0$                              & \multicolumn{1}{lV{3}}{$88.7 \pm 1.1$}                            & $11.8 \pm 2.4$        & $49.6 \pm 1.1$ & $9.0 \pm 1.4$        & $1.6 \pm 1.0$         \\ [0.3cm]
E. 5 & \begin{tabular}[c]{@{}l@{}}task: Pi1-R1 \\ robot: Pu1-R2\end{tabular} & $2.1 \pm 0.4$                                          & $14.7 \pm 2.7$                                        & $4.0 \pm 1.9$                               & \multicolumn{1}{lV{3}}{$9.6 \pm 1.6$}                             & $2.9 \pm 1.0$        & $8.6 \pm 0.3$ & $3.8 \pm 1.6$        & $2.8 \pm 0.9$         \\ [0.3cm]
E. 6 & \begin{tabular}[c]{@{}l@{}}task: Pu1-R3 \\ robot: Pi1-R2\end{tabular} & $8.8 + 1.9$                                          & $55.6 \pm 2.4$                                        & $11.6 \pm 2.0$                              & \multicolumn{1}{lV{3}}{$80.8 \pm 3.4$}                            & $10.5 \pm 2.1$        & $30.5 \pm 4.2$ & $9.0 \pm 0.7$        & $0.1 \pm 0.2$         \\ [0.3cm]
E. 7 & \begin{tabular}[c]{@{}l@{}}task: Pi2-R1 \\ robot: Pi1-R3\end{tabular}  & $4.7 \pm 1.6$                                          & $41.8 \pm 1.7$                                        & $3.6 \pm 0.8$                               & \multicolumn{1}{lV{3}}{$13.1 \pm 2.9$}                            & $3.0 \pm 1.6$        & $9.8 \pm 1.3$ & $3.2 \pm 1.4$        & $0.0 \pm 0.0$         \\ [0.3cm]
E. 8 & \begin{tabular}[c]{@{}l@{}}task: Pi1-R3 \\ robot: Pi2-R1\end{tabular}  & $5.3 \pm 1.7$                                          & $18.4 \pm 1.3$                                        & $3.0 \pm 0.7$                               & \multicolumn{1}{lV{3}}{$18.8 \pm 2.6$}                            & $3.1 \pm 0.5$        & $13.6\pm1.1$ & $3.0 \pm 0.7$        & $0.0\pm0.0$         \\ \hline

\end{tabular}}
\caption{Success rate and touching rate of zero-shot transfer. Our method with relative representation, without relative representation, and the baseline method use the network structures shown in Figure \ref{fig:ours structure}, \ref{fig:ablation structure}, \ref{fig:baseline structure} respectively. The success rate shows the probability of the robot to successfully accomplish the tasks, while the touching rate shows its probability touch the object in the tasks. The first three experiments are easier because the target tasks are easier and the source and target tasks are more similar. In these easier experiments our method achieves significantly higher success rates and touching rates than the baseline. In the other five harder experiments, all the methods have similarly low success rates, but our method still achieves higher touching rates than the baseline.}
\label{zero_shot_rates}
\vskip -0.5cm
\end{table}

==> tables/zero_shot_table_ver7.tex <==
\begin{table}[h]
\footnotesize
\centering
% https://tex.stackexchange.com/questions/39435/how-can-i-center-a-too-wide-table
\addtolength{\leftskip} {-2cm} % increase (absolute) value if needed
\addtolength{\rightskip}{-2cm}
\small
\scalebox{0.9}{
\begin{tabular}{|cccccccccc|}
\hline
        &                                                                                    & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Our method \end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ablation method\end{tabular}} & \multicolumn{2}{c}{Devin et. al. 2017} & \multicolumn{2}{c|}{Baseline method} \\
        &                                                                                    & Success (\%)                                       & Touching(\%)                                      & Success
        (\%)                             & Touching(\%)                                               & Success(\%)      & Touching(\%) & Success(\%)      & Touching(\%)      \\ \hline
E1 & \begin{tabular}[c]{@{}l@{}}t: Pu1-R1 \\ r: Pu2-R2\end{tabular}  & $\boldsymbol{26.9\pm3.6}$                                         & $73.0\pm1.4$                                        & $13.9\pm3.5$                              & \multicolumn{1}{lV{3}}{\boldsymbol{75.8\pm4.4}}                            & $11.7\pm2.6$        & $44.8\pm3.1$ & $6.5\pm2.5$        & $0.0\pm0.0$         \\[0.3cm]
E2 & \begin{tabular}[c]{@{}l@{}}t: Pu2-R1 \\ r: Pu1-R2\end{tabular} & $\boldsymbol{24.4\pm1.5}$                                        & $\boldsymbol{99.9\pm0.2}$                                       & $6.8\pm0.7$                               & \multicolumn{1}{lV{3}}{$93.5\pm2.0$}                            & $10.0\pm0.9$        & $78.3\pm5.4$ & $9.3\pm2.1$        & $17.9\pm2.7$        \\ [0.3cm]
E3 & \begin{tabular}[c]{@{}l@{}}t: Pu1-R3 \\ r: Pu3-R1\end{tabular}   & $\boldsymbol{16.5\pm1.9}$                                         & $90.8\pm2.3$                                        & $7.2\pm1.5$                               & \multicolumn{1}{lV{3}}{$\boldsymbol{95.6\pm0.8}$}                            & $9.8\pm2.5$        & $82.6\pm1.6$ & $8.4\pm3.7$        & $0.0\pm0.0$         \\ [0.3cm] \hlineB{3}
E4 & \begin{tabular}[c]{@{}l@{}}t: Pu3-R1 \\ r: Pu1-R2\end{tabular} & $13.2\pm1.1$                                         & $\boldsymbol{95.4\pm1.9}$                                        & $\boldsymbol{14.9\pm1.0}$                              & \multicolumn{1}{lV{3}}{$88.7 \pm 1.1$}                            & $11.8 \pm 2.4$        & $49.6 \pm 1.1$ & $9.0 \pm 1.4$        & $1.6 \pm 1.0$         \\ [0.3cm]
E5 & \begin{tabular}[c]{@{}l@{}}t: Pi1-R1 \\ r: Pu1-R2\end{tabular} & $2.1 \pm 0.4$                                          & $\boldsymbol{14.7 \pm 2.7}$                                        & $\boldsymbol{4.0 \pm 1.9}$                               & \multicolumn{1}{lV{3}}{$9.6 \pm 1.6$}                             & $2.9 \pm 1.0$        & $8.6 \pm 0.3$ & $3.8 \pm 1.6$        & $2.8 \pm 0.9$         \\ [0.3cm]
E6 & \begin{tabular}[c]{@{}l@{}}t: Pu1-R3 \\ r: Pi1-R2\end{tabular} & $8.8 + 1.9$                                          & $55.6 \pm 2.4$                                        & $\boldsymbol{11.6 \pm 2.0}$                              & \multicolumn{1}{lV{3}}{$\boldsymbol{80.8 \pm 3.4}$}                            & $10.5 \pm 2.1$        & $30.5 \pm 4.2$ & $9.0 \pm 0.7$        & $0.1 \pm 0.2$         \\ [0.3cm]
E7 & \begin{tabular}[c]{@{}l@{}}t: Pi2-R1 \\ r: Pi1-R3\end{tabular}  & $\boldsymbol{4.7 \pm 1.6}$                                          & $\boldsymbol{41.8 \pm 1.7}$                                        & $3.6 \pm 0.8$                               & \multicolumn{1}{lV{3}}{$13.1 \pm 2.9$}                            & $3.0 \pm 1.6$        & $9.8 \pm 1.3$ & $3.2 \pm 1.4$        & $0.0 \pm 0.0$         \\ [0.3cm]
E8 & \begin{tabular}[c]{@{}l@{}}t: Pi1-R3 \\ r: Pi2-R1\end{tabular}  & $\boldsymbol{5.3 \pm 1.7}$                                          & $18.4 \pm 1.3$                                        & $3.0 \pm 0.7$                               & \multicolumn{1}{lV{3}}{$\boldsymbol{18.8 \pm 2.6}$}                            & $3.1 \pm 0.5$        & $13.6\pm1.1$ & $3.0 \pm 0.7$        & $0.0\pm0.0$         \\ \hline

\end{tabular}}
\captionsetup{skip=5pt}
\caption{\textbf{Success rate and touching rate of zero-shot transfer}. 
% Our method with relative representation, without relative representation, and the baseline method use the network structures shown in Figure \ref{fig:ours structure}, \ref{fig:ablation structure}, \ref{fig:baseline structure} respectively. 
% The success rate shows the probability of the robot to successfully accomplish the tasks, while the touching rate shows its probability touch the object in the tasks. 
% The first three experiments are easier because the target tasks are easier and the source and target tasks are more similar. In these easier experiments our method achieves significantly higher success rates and touching rates than the baseline. In the other five harder experiments, all the methods have similarly low success rates, but our method still achieves higher touching rates than the baseline.
The best success and touching rates in each environment are highlighted in bold.
}
\label{zero_shot_rates}
\vskip -0.5cm
\end{table}

==> tables/zero_shot_table_ver8.tex <==
\begin{table}[h]
\setlength\tabcolsep{0pt} % make LaTeX figure out intercolumn whitespace
\caption{\label{Table}Indices}

\begin{tabular*}{\textwidth}{p{1cm} @{\extracolsep{8pt}} rrrrrrrr}
\toprule
\textbf{\textit{Index}}  &   
\multicolumn{4}{c}{\textbf{\textit{Success Rate (\%)}}}  &   
\multicolumn{4}{c}{\textbf{\textit{Touching Rate (\%)}}}  \\
\cmidrule{2-5} \cmidrule{6-9}
& \mc{\textbf{\textit{Ours}}} & \mc{\textbf{\textit{Ablation}}} & \mc{\textbf{\textit{Devin et al.}}} & \mc{\textbf{\textit{Baseline}}} 
& \mc{\textbf{\textit{Ours}}} & \mc{\textbf{\textit{Ablation}}} & \mc{\textbf{\textit{Devin et al.}}} & \mc{\textbf{\textit{Baseline}}}  \\
\midrule
E1               & $\boldsymbol{26.9\pm3.6}$  & $26.9\pm3.6$  & $26.9\pm3.6$  & $26.9\pm3.6$  & $26.9\pm3.6$  & $26.9\pm3.6$  & $26.9\pm3.6$  & $26.9\pm3.6$\\ 
E2               & 0.19\%  & 0.19\%  & 0.21\%  & 0.21\% \\ 
\addlinespace
E1               & 0.06\%  & 0.06\%  & 0.06\%  & 0.06\% \\
E4               & 0.14\%  & 0.14\%  & 0.14\%  & 0.14\% \\ 
E5               & 98.51\% & 98.53\% & 98.51\% & 98.46\%\\ 
\addlinespace
E6               & 0.84\%  & 0.83\%  & 0.85\%  & 0.84\% \\
E7               & 0.70\%  & 0.70\%  & 0.71\%  & 0.71\% \\
E8               & 0.66\%  & 0.66\%  & 0.67\%  & 0.67\% \\
\bottomrule
\end{tabular*}
\end{table}

==> tables/zero_shot_table_ver9.tex <==
% \begin{table}[h]
%     \centering
%     \fontsize{10}{12}\small
%     \begin{tabular}{
%         p{0cm}
%         S[table-format=2.4]
%         @{\extracolsep{10pt}}
%         S[table-format=3.4]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         @{\extracolsep{10pt}}
%         S[table-format=3.1]
%         }
%         \toprule
%         \multicolumn{4}{c}{} & 
%         \multicolumn{2}{c}{Environments}\\
%         \cmidrule(lr){2-9}        
%         & {E1} & {E2} & {E3} & {E4} & {E5} & {E6} & {E7} & {E8}
%         % & {$\lambda$} & {$\psi_e$} & {$\theta_r$} & {$\theta_{sat}$} & {$K_{sat}$} \\ 
%         % & {(-)} & {(\si{cm})} & {(\si{m^3/m^3})} & {(\si{m^3/m^3})} & {(\si{cm/h})} 
%         \\
%         \midrule
%         & \makecell{t: Pu1-R1}  & \makecell{t: Pu2-R1} & \makecell{t: Pu1-R3}& \makecell{t: Pu3-R1}& \makecell{t: Pi1-R1}& \makecell{t: Pu1-R3}&\makecell{t: Pi2-R1}&\makecell{t: Pi1-R3}  \\
%         & \makecell{r: Pu2-R2}  & \makecell{r: Pu1-R2} & \makecell{r: Pu3-R1}& \makecell{r: Pu1-R2}& \makecell{r: Pu1-R2}& \makecell{r: Pi1-R2}&\makecell{r: Pi1-R3}&\makecell{r: Pi2-R1}  \\
%         \bottomrule
%     \end{tabular}
%     \caption{\textbf{Environment description}}
%     \label{table:env-description}
% \end{table}
% \begin{table}[h]
% \setlength\tabcolsep{0pt} % make LaTeX figure out intercolumn whitespace
% \fontsize{10}{12}\small
% \begin{tabular*}{\textwidth}{p{3cm} @{\extracolsep{\fill}} S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)]}
% \toprule
% \multirow{2}{*}{\textbf{\textit{Environments}}} & \multicolumn{4}{c}{\textbf{\textit{Success Rate (\%)}}} \\
% \cmidrule{2-5}
% & {\textbf{\textit{Ours}}} & {\textbf{\textit{Ablation}}} & {\textbf{\textit{Devin et al.}}} & {\textbf{\textit{Baseline}}} \\
% \midrule
% E1               & $\mathbf{26.9 \pm 3.6}$  & $\math{13.9 \pm 3.5}$  & $\math{11.7 \pm 2.6}$  & $\math{6.5 \pm 2.5}$  \\ 
% E2               & $\mathbf{24.4 \pm 1.5}$  & $\math{6.8 \pm 0.7}$  & $\math{10.0 \pm 0.9}$  & $\math{9.3 \pm 2.1}$  \\ 
% E3               & $\mathbf{16.5 \pm 1.9}$  & $\math{7.2 \pm 1.5}$  & $\math{9.8 \pm 2.5}$  & $\math{8.4 \pm 3.7}$  \\ 
% \addlinespace
% E4               & $\math{13.2 \pm 1.1}$  & $\mathbf{14.9 \pm 1.0}$  & $\math{11.8 \pm 2.4}$  & $\math{9.0 \pm 1.4}$  \\ 
% E5               & $\math{2.1 \pm 0.4}$   & $\mathbf{4.0 \pm 1.9}$   & $\math{2.9 \pm 1.0}$   & $\math{3.8 \pm 1.6}$  \\ 
% E6               & $\math{8.8 \pm 1.9}$   & $\mathbf{11.6 \pm 2.0}$  & $\math{10.5 \pm 2.1}$  & $\math{9.0 \pm 0.7}$  \\ 
% E7               & $\mathbf{4.7 \pm 1.6}$   & $\math{3.6 \pm 0.8}$   & $\math{3.0 \pm 1.6}$   & $\math{3.2 \pm 1.4}$  \\ 
% E8               & $\mathbf{5.3 \pm 1.7}$   & $\math{3.0 \pm 0.7}$   & $\math{3.1 \pm 0.5}$   & $\math{3.0 \pm 0.7}$  \\ 
% \bottomrule
% \end{tabular*}
% \caption{\label{Table}\textbf{Success rate of zero-shot transfer}}

% \end{table}
% \vspace{-20pt}
% \begin{table}[h]
% \setlength\tabcolsep{0pt} % make LaTeX figure out intercolumn whitespace
% \fontsize{10}{12}\small
% \begin{tabular*}{\textwidth}{p{3cm} @{\extracolsep{\fill}} S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)]}
% \toprule
% \multirow{2}{*}{\textbf{\textit{Environments}}} & \multicolumn{4}{c}{\textbf{\textit{Touching Rate (\%)}}} \\
% \cmidrule{2-5}
% & {\textbf{\textit{Ours}}} & {\textbf{\textit{Ablation}}} & {\textbf{\textit{Devin et al.}}} & {\textbf{\textit{Baseline}}} \\
% \midrule
% E1               & $\math{73.0 \pm 1.4}$  & $\mathbf{75.8 \pm 4.4}$  & $\math{44.8 \pm 3.1}$  & $\math{0.0 \pm 0.0}$  \\ 
% E2               & $\mathbf{99.9 \pm 0.2}$  & $\math{93.5 \pm 2.0}$  & $\math{78.3 \pm 5.4}$  & $\math{17.9 \pm 2.7}$  \\ 
% E3               & $\math{90.8 \pm 2.3}$  & $\mathbf{95.6 \pm 0.8}$  & $\math{82.6 \pm 1.6}$  & $\math{0.0 \pm 0.0}$  \\ 
% \addlinespace
% E4               & $\mathbf{95.4 \pm 1.9}$  & $\math{88.7 \pm 1.1}$  & $\math{49.6 \pm 1.1}$  & $\math{1.6 \pm 1.0}$  \\ 
% E5               & $\mathbf{14.7 \pm 2.7}$   & $\math{9.6 \pm 1.6}$   & $\math{8.6 \pm 0.3}$   & $\math{2.8 \pm 0.9}$  \\ 
% E6               & $\math{55.6 \pm 2.4}$   & $\mathbf{80.8 \pm 3.4}$  & $\math{30.5 \pm 4.2}$  & $\math{0.1 \pm 0.2}$  \\ 
% E7               & $\mathbf{41.8 \pm 1.7}$   & $\math{13.1 \pm 2.9}$   & $\math{9.8 \pm 1.3}$   & $\math{0.0 \pm 0.0}$  \\ 
% E8               & $\math{18.4 \pm 1.3}$   & $\mathbf{18.8 \pm 2.6}$   & $\math{13.6 \pm 1.1}$   & $\math{0.0 \pm 0.0}$  \\ 
% \bottomrule
% \end{tabular*}
% \caption{\label{Table}\textbf{Touching rate of zero-shot transfer}}

% \end{table}

\begin{table}[t]
\vspace{-5pt}
\setlength\tabcolsep{0pt} % make LaTeX figure out intercolumn whitespace
\fontsize{10}{12}\small
\resizebox{0.97\columnwidth}{!}{
\begin{tabular*}{\textwidth}{p{0.4cm} @{\extracolsep{6pt}} S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)] S[table-format=2.1(2)]}
\toprule
\multirow{2}{*}{\textbf{\textit{}}} & \multicolumn{4}{c}{\textbf{\textit{Touching Rate (\%)}}}  & \multicolumn{4}{c}{\textbf{\textit{Success Rate (\%)}}}\\
\cmidrule{2-5} \cmidrule{6-9} 
& {\textbf{\textit{PS}}} & {\textbf{\textit{PS(Ablation)}}} & {\textbf{\textit{Devin et al.}}} & {\textbf{\textit{Plain}}} & {\textbf{\textit{PS}}} & {\textbf{\textit{PS(Ablation)}}} & {\textbf{\textit{Devin et al.}}} & {\textbf{\textit{Plain}}}\\
\midrule
E1             & $\math{73.0 \pm 1.4}$  & $\mathbf{75.8 \pm 4.4}$  & $\math{44.8 \pm 3.1}$  & $\math{0.0 \pm 0.0}$  & $\mathbf{26.9 \pm 3.6}$  & $\math{13.9 \pm 3.5}$  & $\math{11.7 \pm 2.6}$  & $\math{6.5 \pm 2.5}$  \\ 
E2               & $\mathbf{99.9 \pm 0.2}$  & $\math{93.5 \pm 2.0}$  & $\math{78.3 \pm 5.4}$  & $\math{17.9 \pm 2.7}$  & $\mathbf{24.4 \pm 1.5}$  & $\math{6.8 \pm 0.7}$  & $\math{10.0 \pm 0.9}$  & $\math{9.3 \pm 2.1}$ \\ 
E3               & $\math{90.8 \pm 2.3}$  & $\mathbf{95.6 \pm 0.8}$  & $\math{82.6 \pm 1.6}$  & $\math{0.0 \pm 0.0}$  & $\mathbf{16.5 \pm 1.9}$  & $\math{7.2 \pm 1.5}$  & $\math{9.8 \pm 2.5}$  & $\math{8.4 \pm 3.7}$\\ 
\addlinespace
E4               & $\mathbf{95.4 \pm 1.9}$  & $\math{88.7 \pm 1.1}$  & $\math{49.6 \pm 1.1}$  & $\math{1.6 \pm 1.0}$  & $\math{13.2 \pm 1.1}$  & $\mathbf{14.9 \pm 1.0}$  & $\math{11.8 \pm 2.4}$  & $\math{9.0 \pm 1.4}$\\ 
E5               & $\mathbf{14.7 \pm 2.7}$   & $\math{9.6 \pm 1.6}$   & $\math{8.6 \pm 0.3}$   & $\math{2.8 \pm 0.9}$  & $\math{2.1 \pm 0.4}$   & $\mathbf{4.0 \pm 1.9}$   & $\math{2.9 \pm 1.0}$   & $\math{3.8 \pm 1.6}$\\ 
E6               & $\math{55.6 \pm 2.4}$   & $\mathbf{80.8 \pm 3.4}$  & $\math{30.5 \pm 4.2}$  & $\math{0.1 \pm 0.2}$  & $\math{8.8 \pm 1.9}$   & $\mathbf{11.6 \pm 2.0}$  & $\math{10.5 \pm 2.1}$  & $\math{9.0 \pm 0.7}$ \\ 
E7               & $\mathbf{41.8 \pm 1.7}$   & $\math{13.1 \pm 2.9}$   & $\math{9.8 \pm 1.3}$   & $\math{0.0 \pm 0.0}$ & $\mathbf{4.7 \pm 1.6}$   & $\math{3.6 \pm 0.8}$   & $\math{3.0 \pm 1.6}$   & $\math{3.2 \pm 1.4}$ \\ 
E8               & $\math{18.4 \pm 1.3}$   & $\mathbf{18.8 \pm 2.6}$   & $\math{13.6 \pm 1.1}$   & $\math{0.0 \pm 0.0}$ & $\mathbf{5.3 \pm 1.7}$   & $\math{3.0 \pm 0.7}$   & $\math{3.1 \pm 0.5}$   & $\math{3.0 \pm 0.7}$ \\ 
\bottomrule
\end{tabular*}
}
\caption{\label{Table}\textbf{Success rates and touching rates of zero-shot transfer}}
\label{table:results_zeroshot_sim}
\vspace{-30pt}
\end{table}
